BodyMetric: Evaluating the Realism of Human Bodies in Text-to-Image Generation

Accurately generating images of human bodies from text remains a challenging problem for state of the art text-to-image models. Commonly observed body-related artifacts include extra or missing limbs, unrealistic poses, blurred body parts, etc. Currently, evaluation of such artifacts relies heavily on time-consuming human judgments, limiting the ability to benchmark models at scale. We address this by proposing BodyMetric, a learnable metric that predicts body realism in images. BodyMetric is trained on realism labels and multi-modal signals including 3D body representations inferred from the input image, and textual descriptions. In order to facilitate this approach, we design an annotation pipeline to collect expert ratings on human body realism leading to a new dataset for this task, namely, BodyRealism. Ablation studies support our architectural choices for BodyMetric and the importance of leveraging a 3D human body prior in capturing body-related artifacts in 2D images. In comparison to concurrent metrics which evaluate general user preference in images, BodyMetric specifically reflects body-related artifacts. We demonstrate the utility of BodyMetric through applications that were previously infeasible at scale. In particular, we use BodyMetric to benchmark the generation ability of text-to-image models to produce realistic human bodies. We also demonstrate the effectiveness of BodyMetric in ranking generated images based on the predicted realism scores.

==> bodymetric/components/filtering.tex <==
\begin{table}[h]
\begin{minipage}[b]{0.3\linewidth}
\begin{tabular}{ p{1.8cm}p{1.8cm}}
     \textbf{Vanilla} & \textbf{BodyMetric}  \\
     \multicolumn{2}{p{3.7cm}}{\scriptsize{{a break-dancer defying gravity with flips and spins.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg1/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg1/bodymetric.pdf} \\
     \multicolumn{2}{p{3.8cm}}{\scriptsize{{a model sits casually on a step, legs crossed.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg2/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg2/bodymetric.pdf} \\
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[b]{0.3\linewidth}
\begin{tabular}{ p{1.8cm}p{1.8cm}}
     \textbf{Vanilla} & \textbf{BodyMetric}  \\
    \multicolumn{2}{p{3.7cm}}{\scriptsize{{a male model rests against a motorcycle.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg3/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg3/bodymetric.pdf} \\
    \multicolumn{2}{p{3.7cm}}{\scriptsize{{a hip-hop dancer popping and locking with precision.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg4/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg4/bodymetric.pdf} \\
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[b]{0.3\linewidth}
\begin{tabular}{p{1.8cm}p{1.8cm}}
     \textbf{Vanilla} & \textbf{BodyMetric}  \\
   \multicolumn{2}{p{3.8cm}}{\scriptsize{{a musician performing on stage, lost in the rhythm.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg5/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg5/bodymetric.pdf} \\
   \multicolumn{2}{p{3.8cm}}{\scriptsize{{a jazz dancer improvising with style and flair.}}} \\
   \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg7/random.pdf} &        \includegraphics[width=1.8cm]{bodymetric/figures/filtering/eg7/bodymetric.pdf} \\
\end{tabular}
\end{minipage}\hfill
\captionsetup{type=figure} 
    \caption{Improving text-to-image generation. BodyMetric ranks the generations corresponding to a given text, and selects the image with most realistic representation of human body.}
    \label{fig:sampling}
\end{table}
